Burden in Henselian Valued Fields

In the spirit of the Ax-Kochen-Ershov principle, we show that in certain cases the burden of a Henselian valued field can be computed in terms of the burden of its residue field and that of its value group. To do so, we first see that the burden of such a field is equal to the burden of its RV-sort. These results are generalisations of a work of Chernikov and Simon.

==> Introduction.tex <==
This thesis treats some model theoretical aspects of valued fields. Model theory is a branch of mathematical logic with a focus on the study of algebraic structures and their definable sets. Valued fields are such algebraic structures, that are rich and interesting in many ways. The reader will find below an overview on this topic and a summary of all the main results of this text.


\textbf{Classification theory.}\\
Initiated by the work of Shelah in \cite{She90}, an active area of model theory is the study and the classification of first order theories according to their complexity. The complexity of a theory is measured in terms of combinatorial configurations that it may encode. This is of course a natural idea, that one might find some origin in the famous theorems of Gödel, where the coding abilities of prime numbers are used - revealing at the same time the complexity of the theory of arithmetic. In general, the less a theory is able
to encode complex configurations, the more it is considered as tame. A complex hierarchy of first order theories arises, expressing their relative tameness or complexity. 





\begin{figure}
\begin{center} 
\vspace{-1cm}
\begin{tikzpicture}[line cap=round,line join=round,>=triangle 45,x=1cm,y=1cm,scale=1.0]
\clip(-0.5,-0.5) rectangle (6,6);
\fill[line width=2pt,color=blue,fill=blue,fill opacity=0.3] (0,0) -- (2,0) -- (2,2) -- (0,2) -- cycle;
\fill[line width=2pt,color=blue,fill=blue,fill opacity=0.3] (0,0) -- (4,0) -- (4,2) -- (0,2) -- cycle;
\fill[line width=2pt,color=blue,fill=blue,fill opacity=0.3] (0,0) -- (2,0) -- (2,4) -- (0,4) -- cycle;
\fill[line width=2pt,color=blue,fill=blue,fill opacity=0.3] (0,0) -- (4,0) -- (4,4) -- (0,4) -- cycle;
\draw [line width=2pt,color=black,opacity=0.5] (0,0)-- (4,0) -- (4,4)--(0,4) -- cycle;
\draw [line width=2pt,dashed,color=black,opacity=0.5] (4,0)-- (5,0);
\draw [line width=2pt,dashed,color=black,opacity=0.5] (0,4)-- (0,5);
\draw [line width=2pt,color=black,opacity=0.5] (2,0)-- (2,4);
\draw [line width=2pt,color=black,opacity=0.5] (0,2)-- (4,2);
\draw (3.3,3.3) node { $\text{NTP}_2$};
\draw (3.3,1.3) node {$\text{NIP}$};
\draw (4.5,2) node {$\cdots$};
\draw (1.3,3.3) node {$\text{Simple}$};
\draw (2,4.5) node {$\vdots$};
\draw (1.3,1.3) node {$\text{Stable}$};
\draw (5,5) node {\small $(\mathbb{Z},+,\times)$};
\draw [fill=black] (4.7,4.7) circle (1.5pt);
\draw (3.0,2.5) node {\small $\prod_\mathcal{U} \mathbb{Q}_p$};
\draw [fill=black] (2.4,2.2) circle (1.5pt);
\draw (0.8,2.5) node {\small $\prod_\mathcal{U} \mathbb{F}_p$};
\draw [fill=black] (0.5,2.2) circle (1.5pt);
\draw (2.8,0.5) node {\small $(\mathbb{R},+,\times)$};
\draw [fill=black] (2.4,0.2) circle (1.5pt);
\draw (0.8,0.5) node {\small $(\mathbb{C},+,\times)$};
\draw [fill=black] (0.5,0.2) circle (1.5pt);
\end{tikzpicture}
\vspace{-0.2cm}
\caption*{A classification of first order theories.}
\vspace{-1cm}
\end{center}
\end{figure}
Modern classification of theories started with the study of the class of stable theories; a very tame and undoubtedly an important class of first order theories. A theory is stable if no formula encodes ``$i<j$'' for $i,j\in \mathbb{N}$ (see e.g. \cite{TZ12} for a precise definition). This is a class to which belong the theory of infinite sets, algebraically closed fields and abelian groups. 
Many methods and tools have been specifically developed in order to analyse types
and models, and these have structurally improved our abstract understanding of this class. Let us cite for instance Morley's Categoricity Theorem: if a first-order theory in a countable language is categorical in some uncountable cardinality, then it is categorical in all uncountable cardinalities. This framework has also established deep connections between the geometry of forking independence
and properties of algebraic structures (groups and fields) definable in the
theory. 



However, many natural theories do not fit in this restrictive setting such as any ordered structure, or any `random structure'. After some development, logicians have extended these tools to larger contexts, and have generalised results to some unstable theories. Already in \cite{She90}, two generalisations capturing slightly wilder theories have been defined and studied, namely the class of simple theories (no formula encodes the tree property) -- to which belong the theory of the random graph and the theory of pseudo finite fields -- and the class of $\text{NIP}$ theories (no formula encodes ``$i\in J$'', $i\in \mathbb{N}, J \subset \mathbb{N}$) -- to which belong the theory of real closed fields, of dense linear order, of the field of $p$-adics and of algebraically closed valued fields. These two generalisations are `orthogonal' in the sense that a theory which is both simple and NIP is in fact stable. The interest in these classes grew significantly after some tools and methods developed
for stable theories found interesting extensions to more general contexts
(e.g. see \cite{Sim15} and \cite{KP97}). Ever since, model theory has pushed our knowledge to less and lesser tame theories by generalising these tools to wilder classes. In this conquest of the 'untame land' of first order theories, one of the latest developments concerns the class of $\text{NTP}_2$ theories (no formula encodes the tree property of the second kind). See \cite{CK12} and \cite{Che14}. It appeared to be a particularly interesting generalisation of the class of NIP and Simple theories. For instance, non-principal ultra-products of $p$-adics, the densely ordered random graph, and valued fields with a generic automorphism are $\text{NTP}_2$, but neither simple nor $\text{NIP}$. The main results of this thesis concerns specific $\text{NTP}_2$ theories of valued fields. Before going to details, let us mention instances of other developments in the framework of classification theory:
on one hand, there is the classes of $\text{NSOP}_n$ theories, $n\in \mathbb{N}^\star$,  which form a proper hierarchy of generalisations of simple theories, and which is already meaningful in the study of fields.
On the other hand, the classes of $\text{NIP}_n$ theories (where no formula encodes ``$i\in J$'', $i\in \mathbb{N}^n, J \subset \mathbb{N}^n$) seem to be interesting generalisations of the class of NIP theories, highlighting the importance of combinatorial configurations of higher dimension.


The abstract study of these classes leads to a better understanding
of algebraic structures, as some algebraic phenomena may or not occur,
depending of the complexity of the theory (e.g. \cite{KSW11} and \cite{CKS12}). Of course, the more we study these classes, the more relevant it is to
classify theories. It could be in general a difficult exercise, but many methods are
known: one can show stability (resp.\ NIP) by counting types over small sets
(resp.\ coheirs over models). Simple theories are exactly theories with some
abstract independence relation (\cite{KP97}). The situation is different when
we look at a quantitative version of these notions of complexity. 

\textbf{Quantitative vs Qualitative notions of complexity.} \\
Let us explain what we
mean by `quantitative', or at least, let us give a quick intuition. As we said, a theory is not stable, NIP, nor Simple if instances of a single formula realise a certain combinatorial configuration. For example, the formula $x \vert y $ in the theory of arithmetic, or the formula $x\in y$ in the theory of $\text{ZFC}$ have the strong property to encode the tree property of the second kind, demonstrating that $\text{ZFC}$ and the theory of $(\mathbb{N}, +,\times)$ have $\text{TP}_2$. Even if a theory cannot encode a given combinatorial property, it may however be able to do so partially, and to some extent. And so rises in a certain sense a notion of `rank', or `dimension'. There is probably no recipe which attaches an interesting quantitative notion of complexity to any class of the hierarchy. In our context, one can call `dimension' of a theory the maximal size of sets of formulas $\phi_i(x,y_i)$, such that
a set of $y_i$-instances, called a \textit{pattern}, satisfies the combinatorial configuration. Applied to $\text{NIP}$, this gives us the notion of dp-rank, and applied to $\text{NTP}_2$, the notion of burden, which generalises the former. In particular, we no longer study only the intricacies of instances of one unique formula, but interaction of instances of several formulas.
A major difference between quantitative and qualitative classifications seems to be
the following: though one can use global reasoning in the second case (e.g.\
counting types), one needs however a rather good understanding of formulas in the
first case. A good understanding of formulas could be a synonym for
quantifier elimination, but in practice, one needs an even better
description of one-dimensional definable sets than the one given by quantifier
elimination. Hence, the quantitative classification of first order theories
actually motivates the search for a good description of the definable sets. 
This is of course an important problem on its own, as such a description can
be used for many purposes. 



Computing the burden is indubitably a very active research area
(\cite{Mon17}, \cite{Joh19}, \cite{HP17}). In particular, finite burden or
burden equal to 1 has some relevance (\cite{Adl07}).  A theory of burden one is called \emph{inp-minimal}, or if is $\text{NIP}$,  \emph{dp-minimal}. If it has `non-infinite' burden, it is called \emph{strong}, or if the theory is $\text{NIP}$, \emph{strongly dependent}. 
In model theory of valued fields, it has been shown that the field of
p-adics is dp-minimal (\cite{Dol11},\cite{ADHMS}).  Later in \cite{CS19}, Chernikov and Simon proved that any ultraproduct of the $p$-adics over an
ultrafilter on the prime numbers is inp-minimal, improving Chernikov's earlier
work in \cite{Che14}). As we will see, this computation highlighted some constraint between value group and residue field, with some concrete applications.
\\
\textbf{Stable embeddedness and definability of types}\\
An other important notion present in this text is the notion of stable embeddedness. One can formulate two (equivalent) characterisations of stability: a theory is stable if and only if every complete type is definable if and only if every set is stably embedded.  
In model theory of unstable structures, the notion of stable embeddedness plays an important role. A subset $A$ of an $\mathrm{L}$-structure $\mathcal{M}$ is said to be stably embedded if any intersection of $A$ and of a definable set is the intersection of $A$ and of an $A$-definable set. By a duality between parameters/variables, it is equivalent to say that all types over $A$ are definable over $A$. Understanding stably embedded definable subsets can be a crucial step in order to understand the whole structure. For instance, in the study of Henselian valued fields of equicharacteristic $0$, the value group and residue field are stably embedded substructures that play a primordial role -- we will discuss this fact longer in the introduction. The definition of stably embedded subsets is of course not limited to definable sets and other aspects concern indeed stably embedded submodels of the structure. Given a theory $T$, one can ask: when is a model $\mathcal{M}$ stably embedded in a given elementary extension $\mathcal{N}$? in all elementary extensions? 
One can also ask if this condition is first order: is the class of pairs of model $\mathcal{M} \leq \mathcal{N}$, such that $\mathcal{M}$ is stably embedded in $\mathcal{N}$, axiomatisable in the language of pairs?
By an observation of van den Dries (\cite{VdD86}), being a stably embedded submodel of a real closed field is a first order property in the language of pairs. This was later generalised by Marker and Steinhorn to any o-minimal theories. They in fact prove that any $o$-minimal structure over which all $1$-types are definable has all types definable. Few other structures satisfy analogous property, such as Presburger arithmetic and the theory of random graphs. Let us now introduce the structures that we mainly studied in this text, namely the valued fields. 




%In the model theory of Henselian valued fields, a common approach follows the
%philosophy behind the Ax-Kochen-Er\v{s}hov principle: to compare the complexity of
%a valued field with that of the residue field and that of the value group. A
%theorem of Delon \cite{Del81} is the first instance of this: a Henselian
%valued field of equicharacteristic 0 is NIP if and only if both its residue
%field and its value group are NIP. The main aspect of my thesis consists of determining the burden of various theories of valued fields, in terms of the burden of the value group and that of the residue fields.




\textbf{Valued fields.}\\
Many fields are naturally endowed with a valuation such as the field of formal power series $K((t))$ over a field $K$ or the field of $p$-adics numbers $\mathbb{Q}_p$ for a prime $p$. Valued fields are rich algebraic structures and are very well studied in the framework of algebraic number theory, algebraic geometry and also model theory. In particular, model theorists found in the theory of valued fields a rich source of applications. Let us mention for instance the Denef rationality results for Poincaré series, the foundations of motivic integration and the Ax-Kochen-Er\v{s}hov principle -- bringing the study of valued fields in the scope of model theory. %Furthermore, Henselian valued fields appear to be a perfect playground for deep model theoretic considerations.$\mathcal{U}$ is a non-principal ultra-filter on the set on primes number, then the ultra-product $\Pi_{\mathcal{U}}\mathbb{Q}_p$

%Real closed fields with the infinetesimal valuation or the fields of $p$-adics with the $p$-adic valuation. The latest being definable in the language of fields.


In the study of a valued field $\mathcal{K}$, the value group $\Gamma$ and the residue field $k$ play important roles, as we said. In the case that we will study, they will be always stably embedded substructures. It is often useful to consider a valued field as a leveled tree branching $\vert k \vert$-many times in $\vert \Gamma \vert$-many levels. It gives a picture for the valuation of an element or of the difference of two elements. The topology also becomes more intuitive. However, it fails to represent the field structure, in particular the multiplication. Nonetheless, it appears very useful in the context of this text. The reader will find some of these representations to support the intuition. We leave here a representation of the field $\mathbb{Q}_3$ of $3$-adics, as an example.\\
    
\begin{center}
\begin{minipage}{0.70\linewidth}

    
    \definecolor{zzttqq}{rgb}{0.6,0.2,0.}
\begin{tikzpicture}[line cap=round,line join=round,>=triangle 45,x=1.0cm,y=1.0cm]
\clip(7.4404953018657027,-2.5491252321245788) rectangle (22.246788671250542,7.9806684556859375);
\fill[line width=1.2pt,color=zzttqq,fill=zzttqq,fill opacity=0.10000000149011612] (13.5,5.) -- (13.218813038658245,7.) -- (13.806700277899749,7.) -- cycle;
\draw [line width=1.2pt,dash pattern=on 2pt off 2pt] (16.,5.)-- (18.,7.);
\draw [line width=1.2pt] (12.,1.)-- (11.5,3.);
\draw [line width=1.2pt] (12.,1.)-- (12.5,3.);
\draw [line width=1.2pt] (14.,3.)-- (13.5,5.);
\draw [line width=1.2pt] (14.,3.)-- (14.5,5.);
\draw [line width=1.2pt] (11.5,3.)-- (11.2,5.);
\draw [line width=1.2pt] (11.5,3.)-- (11.5,5.);
\draw [line width=1.2pt] (11.5,3.)-- (11.8,5.);
\draw [line width=1.2pt] (12.5,3.)-- (12.2,5.);
\draw [line width=1.2pt] (12.5,3.)-- (12.5,5.);
\draw [line width=1.2pt] (12.5,3.)-- (12.8,5.);
\draw [line width=1.2pt] (9.99959147998603,-1.000408520014005)-- (9.499591479986028,0.9995914799859937);
\draw [line width=1.2pt] (9.99959147998603,-1.000408520014005)-- (10.49959147998603,0.9995914799859942);
\draw [line width=1.2pt] (9.499591479986028,0.9995914799859937)-- (9.19959147998602,2.9995914799859875);
\draw [line width=1.2pt] (9.499591479986028,0.9995914799859937)-- (9.499591479986021,2.9995914799859875);
\draw [line width=1.2pt] (9.499591479986028,0.9995914799859937)-- (9.799591479986022,2.9995914799859875);
\draw [line width=1.2pt] (10.49959147998603,0.9995914799859942)-- (10.19959147998602,2.9995914799859875);
\draw [line width=1.2pt] (10.49959147998603,0.9995914799859942)-- (10.499591479986021,2.9995914799859875);
\draw [line width=1.2pt] (10.49959147998603,0.9995914799859942)-- (10.799591479986022,2.9995914799859875);
\draw [line width=1.2pt] (9.19959147998602,2.9995914799859875)-- (9.099707001451604,5.);
\draw [line width=1.2pt] (9.19959147998602,2.9995914799859875)-- (9.310147551983366,5.);
\draw [line width=1.2pt] (9.19959147998602,2.9995914799859875)-- (9.2,5.);
\draw [line width=1.2pt] (9.499591479986021,2.9995914799859875)-- (9.4,5.);
\draw [line width=1.2pt] (9.499591479986021,2.9995914799859875)-- (9.49750630322503,5.);
\draw [line width=1.2pt] (9.6,5.)-- (9.499591479986021,2.9995914799859875);
\draw [line width=1.2pt] (9.799591479986022,2.9995914799859875)-- (9.703351767379768,5.);
\draw [line width=1.2pt] (9.799591479986022,2.9995914799859875)-- (9.8,5.);
\draw [line width=1.2pt] (9.799591479986022,2.9995914799859875)-- (9.89992633658595,5.);
\draw [line width=1.2pt] (10.19959147998602,2.9995914799859875)-- (10.10014117559224,5.);
\draw [line width=1.2pt] (10.19959147998602,2.9995914799859875)-- (10.2,5.);
\draw [line width=1.2pt] (10.19959147998602,2.9995914799859875)-- (10.300356014598533,5.);
\draw [line width=1.2pt] (10.499591479986021,2.9995914799859875)-- (10.50421112340494,5.);
\draw [line width=1.2pt] (10.499591479986021,2.9995914799859875)-- (10.4,5.);
\draw [line width=1.2pt] (10.499591479986021,2.9995914799859875)-- (10.6,5.);
\draw [line width=1.2pt] (10.799591479986022,2.9995914799859875)-- (10.8,5.);
\draw [line width=1.2pt] (10.799591479986022,2.9995914799859875)-- (10.904640801417525,5.);
\draw [line width=1.2pt] (10.799591479986022,2.9995914799859875)-- (10.700785692611118,5.);
\draw [line width=1.2pt,dash pattern=on 2pt off 2pt] (9.099707001451604,5.)-- (8.798268831271011,7.);
\draw [line width=1.2pt,dash pattern=on 2pt off 2pt] (9.2,5.)-- (9.198576162247367,7.);
\draw [line width=1.2pt,dash pattern=on 2pt off 2pt] (9.310147551983366,5.)-- (9.605885006268819,7.);
\draw [line width=1.2pt,dash pattern=on 2pt off 2pt] (11.2,5.)-- (11.,7.);
\draw [line width=1.2pt,dash pattern=on 2pt off 2pt] (11.5,5.)-- (11.52212658332249,7.);
\draw [line width=1.2pt,dash pattern=on 2pt off 2pt] (12.2,5.)-- (12.,7.);
\draw [line width=1.2pt,color=zzttqq] (13.5,5.)-- (13.218813038658245,7.);
\draw [line width=1.2pt,color=zzttqq] (13.218813038658245,7.)-- (13.806700277899749,7.);
\draw [line width=1.2pt,color=zzttqq] (13.806700277899749,7.)-- (13.5,5.);
\draw [line width=2.4pt,color=zzttqq] (13.218813038658245,7.)-- (13.806700277899749,7.);
\draw (9.726827791585928,0.7788984261624499) node[anchor=north west] { $\mathbb{F}_3^\times$};
\draw (8.749836624675682,2.5680823372020934) node[anchor=north west] {	        $k=\mathbb{F}_3$};
\draw (17.162816117513902,7.872113881584799) node[anchor=north west] {$\mathbb{Q}_3$};
\draw (16.240102237654224,4.543106942483192) node[anchor=north west] {$\Gamma=\mathbb{Z}$};
\draw (17.940790565238725,6.858937856640831) node[anchor=north west] {$\infty$};
\draw [line width=1.2pt] (7.,7.)-- (18.,7.);
\draw [line width=1.2pt,dotted] (7.,5.)-- (18.,5.);
\draw [line width=1.2pt,dotted] (18.,2.9995914799859875)-- (7.,2.9995914799859875);
\draw [line width=1.2pt,dotted] (7.,0.9995914799859925)-- (18.,0.9995914799859976);
\draw [line width=1.2pt,dotted] (18.,-1.)-- (7.,-1.);
\draw [line width=1.2pt] (9.,-2.)-- (16.,5.);
\draw [line width=1.2pt,dash pattern=on 2pt off 2pt] (9.,-2.)-- (8.,-3.);
\begin{scriptsize}
\draw [fill=black] (16.,5.) circle (1.0pt);
\draw [fill=black] (18.,7.) circle (1.5pt);
\draw[color=black] (18.23026942950843,7.266017509520103) node {$0$};
\draw [fill=black] (12.,1.) circle (1.0pt);
\draw [fill=black] (11.5,3.) circle (1.5pt);
\draw[color=black] (11.186100188594573,2.7614943247301097) node {$\rv_0(3)$};
\draw [fill=black] (12.5,3.) circle (1.0pt);
\draw [fill=black] (13.5,5.) circle (1.0pt);
\draw [fill=black] (14.5,5.) circle (1.0pt);
\draw [fill=black] (11.2,5.) circle (1.0pt);
\draw [fill=black] (11.5,5.) circle (1.0pt);
\draw [fill=black] (11.8,5.) circle (1.0pt);
\draw [fill=black] (12.2,5.) circle (1.0pt);
\draw [fill=black] (12.5,5.) circle (1.0pt);
\draw [fill=black] (12.8,5.) circle (1.0pt);
\draw [fill=black] (11.99959147998603,0.9995914799859948) circle (1.5pt);
\draw[color=black] (12.40450728608067,0.5899112023000339) node {$1$};
\draw [fill=black] (9.99959147998603,-1.000408520014005) circle (1.5pt);
\draw[color=black] (10.522894668327607,-1.3278862734867611) node {$0$};
\draw [fill=black] (9.499591479986028,0.9995914799859937) circle (1.5pt);
\draw[color=black] (8.921714700335817,0.6170498458253189) node {$\rv_0(1)$};
\draw [fill=black] (10.49959147998603,0.9995914799859942) circle (1.0pt);
\draw [fill=black] (9.19959147998602,2.9995914799859875) circle (1.5pt);
\draw[color=black] (8.415126687863838,2.788141327848106) node {$\rv_1(2)$};
\draw [fill=black] (9.499591479986021,2.9995914799859875) circle (1.0pt);
\draw [fill=black] (9.799591479986022,2.9995914799859875) circle (1.0pt);
\draw [fill=black] (10.19959147998602,2.9995914799859875) circle (1.0pt);
\draw [fill=black] (10.499591479986021,2.9995914799859875) circle (1.0pt);
\draw [fill=black] (9.099707001451604,5.) circle (1.5pt);
\draw[color=black] (8.415126687863838,4.687846374618044) node {$\rv_2(1)$};
\draw [fill=black] (9.310147551983366,5.) circle (1.0pt);
\draw [fill=black] (9.2,5.) circle (1.0pt);
\draw [fill=black] (9.4,5.) circle (1.0pt);
\draw [fill=black] (9.49750630322503,5.) circle (1.0pt);
\draw [fill=black] (9.6,5.) circle (1.0pt);
\draw [fill=black] (9.703351767379768,5.) circle (1.0pt);
\draw [fill=black] (9.8,5.) circle (1.0pt);
\draw [fill=black] (9.89992633658595,5.) circle (1.0pt);
\draw [fill=black] (10.10014117559224,5.) circle (1.0pt);
\draw [fill=black] (10.2,5.) circle (1.0pt);
\draw [fill=black] (10.300356014598533,5.) circle (1.0pt);
\draw [fill=black] (10.50421112340494,5.) circle (1.0pt);
\draw [fill=black] (10.4,5.) circle (1.0pt);
\draw [fill=black] (10.6,5.) circle (1.0pt);
\draw [fill=black] (10.8,5.) circle (1.0pt);
\draw [fill=black] (10.904640801417525,5.) circle (1.0pt);
\draw [fill=black] (10.700785692611118,5.) circle (1.0pt);
\draw [fill=black] (8.798268831271011,7.) circle (1.5pt);
\draw[color=black] (8.496542618439692,7.465034228705526) node {$1$};
\draw [fill=black] (9.198576162247367,7.) circle (1.5pt);
\draw[color=black] (9.093592775995955,7.465034228705526) node {$1+3^2$};
\draw [fill=black] (9.605885006268819,7.) circle (1.5pt);
\draw[color=black] (10.187693091108475,7.465034228705526) node {$1+2\cdot 3^2$};
\draw [fill=black] (11.,7.) circle (1.5pt);
\draw[color=black] (10.970928106698447,7.465034228705526) node {$3$};
\draw [fill=black] (11.52212658332249,7.) circle (1.5pt);
\draw[color=black] (11.654163122288422,7.465034228705526) node {$3+3^2$};
\draw [fill=black] (12.,7.) circle (1.5pt);
\draw[color=black] (12.421616434282949,7.465034228705526) node {$2\cdot 3$};
\draw [fill=black] (13.218813038658245,7.) circle (1.5pt);
\draw[color=black] (13.30912873692349,7.46773660840378) node {$3^2$};
\draw [fill=black] (13.806700277899749,7.) circle (1.5pt);
\draw[color=black] (14.629876055154007,7.467773660840378) node {$3^2+2\cdot 3^3$};
\draw[color=zzttqq] (14.66193110275219,6.256971295011676) node {$B_{>3}(3^2)$};
\draw [fill=black] (14.,3.) circle (1.5pt);
\draw[color=black] (14.304212332850591,2.670540539238538) node {$2$};
\end{scriptsize}
\end{tikzpicture}


\end{minipage}
\end{center}



\textbf{The Ax-Kochen-Er\v{s}hov principle and `benign' theories.}\\
As usual in mathematics, one can prove relative results, and in the context
of the classification, it can take the following form: understanding the
complexity of a structure in term of that of a simpler substructure. The theory of valued fields is a fruitful playground for this `philosophy' with 
the transfer principle of Ax-Kochen-Er\v{s}hov, discovered by Ax and Kochen (\cite{AK65A}, \cite{AK65B}, \cite{AK66}) and independently by Er\v{s}hov (\cite{Ers65A}, \cite{Ers65C},\cite{Ers65B},\cite{Ers65D},\cite{Ers66},\cite{Ers67A},\cite{Ers67B}). 
This principle states that the theory of Henselian valued fields of equicharacteristic $0$ is completely determined by the theory of its residue field and that of its value group. One deduces from it the
celebrated transfer principle between $\mathbb{F}_p((t))$ and
$\mathbb{Q}_p$ for $p$ large enough, and the approximate solution of Artin's conjecture. It has been shown that many theories are model complete relative to the
residue field and the value group, such as
    \begin{enumerate}
        \itemsep-0.1cm
        \item Henselian valued fields of characteristic $(0,0)$,
        \item algebraically closed valued fields, 
        \item algebraically maximal Kaplansky valued fields.
%        \item unramified mixed characteristic Henselian valued fields with perfect residue fields.
    \end{enumerate}
    Notice that all these fields are Henselian - meaning that in these fields, a Newton process for extracting roots is possible. Although it is an important algebraic property -- and moreover a first order one -- we will rarely use explicitly its definition. %/!/check H-minimality clucker  Halupczok /!/
However it will be implicitly used through the assumption of relative quantifier elimination. It is an important model theoretic property with a well known consequence that we discussed earlier: these valued fields enjoy the property that their residue fields (resp.\ value groups) are stably embedded and pure, in the sense that all sets definable in the residue field (resp.\ value group) may be defined in the language of fields (resp.\ ordered abelian group) with parameters in the residue field (resp.\ value group). In this text, we will refer to the theories listed above as \textit{benign} theories of Henselian valued fields, as they behave nicely for the point of view of model theory.   
 In Subsection \ref{Preliminaries Benign theory of Henselian valued fields}, we will isolate few others important model theoretic properties that these theories of valued fields share and keep track of when they are used. The goal is to implicitly work axiomatically, and to emphasise model theoretic assumptions rather than algebraic ones. %Then, the reader aware of recent development on model theory of valued fields will be able to complete this list themself. 

One may be tempted to add to this list the theory of unramified Henselian valued fields of mixed characteristics with perfect residue field. We have indeed a result of Bélair in \cite{Bel99} who showed the model completeness relative to the value group and residue field\footnote{It has been improved recently by Jahnke and Ascombe, who no longer assume the residue field to be perfect.}. However the theory have some specificity -- fortunately not too challenging. It will be treated in different paragraphs, as it needs different tools and observations. See the paragraph in Subsection \ref{Preliminaries Unramified mixed characteristic Henselian valued fields} for mixed characteristic valued fields.  

These `benign' Henselian valued fields are opposed to wilder fields, such as $\mathbb{F}_p((t))$, which is Henselian but where an Ax-Kochen-Er\v{s}hov-like principle does not hold. In fact, a complete axiomatisation of $\mathbb{F}_p((t))$ is yet unknown: Kuhlmann showed that a natural set of axioms is not sufficient (\cite{Kuh01}). This is an active problem, and recent progress has been made concerning its existential theory (\cite{AF16}).

We will prove two distinct transfer principles for these benign valued fields and unramified mixed characteristic Henselian valued fields with perfect residue field. The first concerns its complexity with respect to the burden: What is the burden of such a valued field in terms of burden of its residue field and value group?
The second concerns stably embedded elementary extensions of such fields: when is such a valued field stably embedded in an elementary extension?
These two distinct questions are united by the fact that they can be approached by similar methods. We will discuss these methods after stating all the main results.


\textbf{Transfer principles for burden.}\\
One can expect, in principle, to understand the complexity of benign theories relatively to that of the value group and that of the residue field. 
A theorem of Delon \cite{Del81} is the first instance of this approach in the context of the classification theory: a Henselian
valued field of equicharacteristic 0 is NIP if and only if both its residue field and its value group are NIP\footnote{It was later showed by Gurevich and Schmitt that any pure ordered abelian group is NIP.}. A more quantitative transfer in $\text{NIP}$ Henselian valued fields was then showed by Shelah in \cite{She14}: a Henselian valued field of equicharacteristic 0 is strongly dependent if and only if both its residue field and its value group are strongly dependent. Both results were generalised to $\text{NTP}_2$ theories by Chernikov in \cite{Che14}: a Henselian valued field of equicharacteristic 0 is $\text{NTP}_2$ (resp.\ strong, of finite burden) if and only if both of its residue field and its value group are $\text{NTP}_2$\footnote{(This theorem failed in general. It has been shown that $\mathbb{F}_p((t))$ has $\text{TP}_2$, while its value group and residue field are $\text{NTP}_2$. See \cite{CKS12}).}(resp.\ strong, of finite burden).
Then, there is a finer result of Chernikov and Simon: consider a Henselian valued field of characteristic $(0,0)$. Assume the residue field $k$ satisfies
    \begin{equation}
            \tag{$H_{k}$} k^\star/(k^\star)^p \ \text{is finite for every prime p.}
    \end{equation}
Then the Henselian valued field of equicaracteristic 0 and residue field $k$ is inp-minimal (\textit{i.e.} of burden one) if and only if the residue field and the value group are both inp-minimal.
They deduced the fact cited earlier: any ultraproduct $\Pi_{\mathcal{U}} \mathbb{Q}_p$ of the $p$-adics (over an ultrafilter $\mathcal{U}$ on the prime numbers)
is inp-minimal. Interestingly, this result particularly echoes the original transfer principle of Ax-Kochen-Er\v{s}hov: the later indeed takes place in such an ultraproduct, and a good understanding of this structure is by consequence a long term goal. 
As many rank/dimension 1 version of complexity (strongly-minimal, SU-rank 1 etc.), this notion plays an important role. Let us cite the classification of dp-minimal fields \cite{Joh15}, and of dp-minimal valued fields \cite{JSW}. It has been shown that dp-minimal ordered abelian groups $(\Gamma,+,0,<)$ are exactly the \emph{non-singular ones} (\cite{JSW}), meaning that $\Gamma/p\Gamma$ is finite for all prime $p$. A natural question is then to consider the classification of valued fields of higher burden. 
This naturally requires generalisations of Chernikov and Simon's theorem. One can ask, as they did in \cite[Problem 26]{CS19}, the following question: Given a Henselian valued field $\mathcal{K}$ of equicharacteristic $0$, with residue field of burden $n$ and value group of burden $m$. Can we compute burden of $\mathcal{K}$?
We give a full answer to this question. Recall that, for us, a `benign' Henselian valued field is either of equicharacteristic $0$, algebraically closed or algebraically maximal Kaplansky.

{
    \renewcommand{\thetheorem}{\ref{ThmBdnHenValFieCha00}}
    \begin{theorem}
        Let $\mathcal{K}=(K, \Gamma, k)$ be a benign Henselian valued field, with value group $\Gamma$ and residue field $k$. Then: 
        \[\bdn(\mathcal{K})= \max_{n\geq 0} \left(\bdn(k^\star/{k^\star}^n) + \bdn (n\Gamma) \right).\]
    \end{theorem}
    \addtocounter{theorem}{-1}
}   
   
It justifies \textit{a postiori} the hypothesis in Chernikov-Simon's theorem, and shows that it is an optimal statement: an equicharacteristic 0 Henselian Non-trivially valued field with inp-minimal value group and inp-minimal residue field is inp-minimal if and only if the residue field satisfies ($H_{k}$). This answers at the same time \cite[Problem 25]{CS19}.

The formula in itself as well as the proof shows a certain constrain between the value group and residue field within the valued field. 
In some sense, it behaves --in terms of complexity-- like in a disjoint union structure $\Gamma \cup k$, rather than in a product structure $\Gamma \times k$. Hopefully, this should give some indication and intuition for future research in the classification of Henselian valued fields, where this distinction will be probably relevant. 

Naturally, we can also consider a Henselian valued field with an angular component, \textit{i.e.} a multiplicative map which associates to every element of the valued field a coefficient in the residue field and which coincides with the residue map on elements of value $0$. We obtain:

    {
    \renewcommand{\thetheorem}{\ref{ThmBdnHenselianValuedFieldequicaracteristicAngularComponent}}
    \begin{theorem}
    Let $\mathcal{K}_{\ac}=(K, \Gamma, k, \ac)$ be a benign Henselian valued field endowed with an $\ac$-map $\ac$, with value group $\Gamma$ and residue field $k$. Then:
    $\bdn(\mathcal{K}_{\ac})= \bdn(k)+ \bdn(\Gamma)$.
    \end{theorem}
    
    \addtocounter{theorem}{-1}
    }

The study of valued fields without $\ac$-map provide \textit{a priori} finer results, but it is interesting to notice that the behavior changes -- the complexity is now similar to that of the product structure $k \times \Gamma$ -- and it is due to a simple reason that we going to make clear in this text. This difference yields for instance to the impossibility to define uniformly in $p$ an angular component in the fields of $p$-adics (see Subsection \ref{subsubsac}), or in general, to the impossibility to define an $\ac$-map in certain Henselian valued fields (see remark \ref{CorollaryNoDefinableAngularComponent}).

For unramified inequal characteristic Henselian valued fields with perfect residue field, we have the following:
    {
    \renewcommand{\thetheorem}{\ref{theoremmixedchar}}
    \begin{theorem}
        Let $\mathcal{K}=(K,k,\Gamma)$ be an unramified mixed characteristic Henselian valued field  with value group $\Gamma$ and residue field $k$. We denote by $\mathcal{K}_{\ac_{<\omega}}=(K,k,\Gamma,\ac_n,n<\omega)$ the structure $\mathcal{K}$ endowed with compatible $\ac$-maps. Assume that the residue field $k$ is perfect. One has 
        \[\bdn(\mathcal{K})= \bdn(\mathcal{K}_{\ac_{<\omega}})= \max(\aleph_0 \cdot \bdn(k), \bdn(\Gamma)).\]
    \end{theorem}
    \addtocounter{theorem}{-1}
    }
Notice that this time, there is no difference between valued fields and valued fields endowed with $\ac$-maps (maps with a plural, as it refers in this context to countably many maps. See \ref{DefinitionAngularComponentsMixedCharacteristic}). Notice that the multiplication sign between the two cardinals $\aleph_0 \cdot \bdn(k)$ cannot be replaced by an addition or a max, as we have to consider finite fields (of burden $0$)\footnote{Another reason is that $k$ can for example be of burden `$\aleph_{\omega-}$'. See Subsection \ref{More on burden and strongness}.}.
It follows that the ring of Witt vectors $W(\mathbb{F}_p^{alg})$ -- in fact any unramified inequal characteristic Henselian valued field with \emph{infinite} perfect residue field -- is not strong. This is perceived as a negative result. 


We now describe our second type of transfer principles.\\

\textbf{Transfer principle for definability of types.}\\
As we said earlier, stably embedded elementary pairs of real closed fields form an elementary class in the language of pairs ((\cite{VdD86})).  Motivated by a similar question, Cubides and Delon have shown in \cite{CD16} that an algebraically closed valued field $\mathcal{K}$ is stably embedded in an elementary extension  $\mathcal{L}$ if and only if the valued fields extension $\mathcal{K} \preceq \mathcal{L}$ is \textit{separated} (see Definition \ref{DefinitionSeparated}) and the small value group $\Gamma_K$ is stably embedded in the larger value group $\Gamma_L$. Recently, Cubides and Ye proved in \cite{CY19} a similar statement for p-adically closed valued fields and real closed valued fields. We give in this text a generalisation to benign Henselian valued fields.
    In fact, we give two statements:

{
    \renewcommand{\thetheorem}{\ref{TheoremReductionGammakElementaryPairs}}
    \begin{theorem}
    Assume that $T$ is a benign theory of Henselian valued fields. 
    Let $\mathcal{K} \preceq \mathcal{L}$ be an elementary pair of models of $T$. The following are equivalent:
        \begin{enumerate}
            \item $\mathcal{K}$ is (uniformly)\footnote{We distinguish in this text two natural notions of stable embeddedness/definability of types: the uniform and non-uniform one. See Definitions \ref{DefinitionStableEmbeddness} and \ref{DefUniStaEmb}.} stably embedded in $\mathcal{L}$, 
            \item The extension $\mathcal{L}/\mathcal{K}$ is separated, the residue field of $\mathcal{K}$ is (uniformly) stably embedded in the residue field of $\mathcal{L}$ and the value group of $\mathcal{K}$ is (uniformly) stably embedded in the value group of $\mathcal{L}$.
        \end{enumerate}
    \end{theorem}
    \addtocounter{theorem}{-1}
}   

    Even if in practice, we will mainly consider elementary extensions of benign valued fields as the situation is simpler (see Subsection \ref{PreliminariesOnDefinableTypes}), we consider in the second statement non-elementary extensions of valued fields, in order to enlarge the scope of applications: 
    
    {
\renewcommand{\thetheorem}{\ref{TheoremReductionGammakNonElementaryPairs}}
    \begin{theorem}%correction
    Assume that $T$ is a benign theory of Henselian valued fields. 
    Let $\mathcal{L}/ \mathcal{K}$ be a separated extension of valued fields with $\mathcal{L}\models T$. 
    Assume either
    \begin{itemize}
            \item that the value group of $\mathcal{K}$ is a pure subgroup of the value group of $\mathcal{L}$,
            \item or that the multiplicative group of the residue field $k_L$ of $\mathcal{L}$ is divisible. %$k_L^\star/(k_L^\star)^n$ is trivial for all $n\geq 1$. 
    \end{itemize}
    
    The following are equivalent:
    
        \begin{enumerate}
            \item $K$ is stably embedded (resp.\ uniformly stably embedded) in $\mathcal{L}$,
            \item the residue field of $\mathcal{K}$ is stably embedded (resp.\ uniformly stably embedded) in the residue field of $\mathcal{L}$ and the value group of $\mathcal{K}$ is stably embedded (resp.\ uniformly stably embedded) in the value group of $\mathcal{L}$.
        \end{enumerate}
    \end{theorem}
\addtocounter{theorem}{-1}
}

    In particular, the field of $p$-adics $\mathbb{Q}_p$ is stably embedded in $\mathbb{C}_p$, the completion of its algebraic closure. 
    
    Again, with some additional observation, one can adapt these arguments and treat the case of unramified mixed characteristic Henselian valued fields with perfect residue field. We show indeed a similar statement for elementary pairs:

{
\renewcommand{\thetheorem}{\ref{TheoremReductionGammakElementaryPairsMixeCharacteristic}}
    \begin{theorem} 
        Let $\mathcal{K}$ be a unramified mixed characteristic Henselian valued field with perfect residue field and $\mathcal{L}$ be an elementary extension. The following are equivalent:
        \begin{enumerate}
            \item $\mathcal{K}$ is stably embedded (resp.\ uniformly stably embedded) in $\mathcal{L}$;
            \item The extension $\mathcal{L}/\mathcal{K}$ is separated, the residue field of $\mathcal{K}$ is stably embedded (resp.\ uniformly stably embedded) in the residue field of $\mathcal{L}$ and the value group of $\mathcal{K}$ is stably embedded (resp.\ uniformly stably embedded) in the value group of $\mathcal{L}$.
        \end{enumerate}
    \end{theorem}
    \addtocounter{theorem}{-1}
}


Also interesting is of course the method to prove these results. It is largely inspired by a method used in \cite{CS19}, which take source from well-known algebraic considerations. We will briefly summarise in these lines, but let us first discuss the limits of a direct approach. \\

\textbf{Limit of the theorem of Pas}.\\
In the setting of Henselian valued fields of characteristic
$(0,0)$, a very important tool is the theorem of Pas: Henselian valued fields
of characteristic $(0,0)$ endowed with an angular component eliminate field-sorted quantifiers. From this powerful result, one deduces easily the
Ax-Kochen-Er\v{s}hov principle. However, it is insufficient in our context, as
adding an ac-map to the language generates more structure and for instance more
opportunities to partially encode the tree property of the second kind. This is indeed
what happens: we show that the burden of a non-principal
ultraproduct of p-adics endowed with an ac-map is equal to 2.
Instead of using the theorem of Pas, Chernikov and Simon proceed with an
intermediate step: before reducing to the residue field and value group,
they consider another interpretable sort, the RV-sort. This is a rather unusual
structure, highly relevant in the study of valued fields.% (probably standing for Residue-Valuation).





\textbf{History of the RV-sort.}\\
First traces of an intermediate structure between the valued field and the
residue field and value group, can be found in a note of Krasner \cite{Kra44}.
This idea has been brought to the scope of model theory by Basarab
(\cite{Bas91}). After successive modifications  (\cite{Kuh94}), Flenner
 came up with the current definition of the RV-sort \cite{Fle11}. The $\RV$-sort of a 
valued field $K$ is the structure $K^\star/(1+\mathfrak{m})$ where $\mathfrak{m}$ is
the maximal ideal of the valuation ring. We denote by $\rv$ the natural
projection. The $\RV$-sort offers an additional point of view: let us cite Hrushovski and Kazdan's work in motivic integration \cite{HK06}, where RV-sort are used, as opposed to Denef, Loeser and Cluckers' work \cite{CL04A}, \cite{CL04B}, \cite{DL01}  where ac-maps are used.




Benign theories of Henselian valued field also eliminate quantifiers relatively to the $\RV$-sort. Similarly to the value group and residue field, one sees that the $\RV$-sort is stably embedded and pure, and can be considered as an autonomous structure. Its full structure is induced by the exact sequence of abelian
groups
\[1 \rightarrow k^\star \rightarrow \RV \rightarrow  \Gamma \rightarrow 0\]
where $k^\star$ is the multiplicative group of the residue field, and
$\Gamma$ is the value (ordered abelian) group. It is also possible to
consider it as a one-sorted structure $(\RV,\cdot, \oplus)$ where $\cdot$
is the group multiplication and $\oplus$ is some sort of non-associative
addition, extending the addition of $k$ (also defined in \cite{Fle11}). 

 
One point of view, defended for instance in \cite{Fle11}, would be to consider $\RV$-sorts as stand alone structures, interesting on their own (as fields and groups are). Reduction principles to the $\RV$-sort would be of equal importance, or could replace classical reduction principles to value group and residue field. 
A good understanding of some aspect of the $\RV$-sort is indeed a crucial step in all the theorems above. In algebra of valued fields, traditional proofs require a distinction between three kind of extension: ramified (new value in the value group), residual (new elements in the residue field) and immediate extension (no new value and no new residue).
Considering analogous statements for the $\RV$-sort, one would have to only distinguish immediate and non-immediate extensions. But it is a complicated algebraic object, containing an ordered abelian group and a field. Adapting all classical statements of the algebra of valued fields from the point of the $\RV$-sort requires some work, and it is not clear that algebraists will gain to do so. But towards this idea, the reader will find some results in this text. We produce in Appendix \ref{AxiomatisationRV} an axiomatisation of $\RV$ and show that all such $\RV$-structures are the $\RV$-sort of a Henselian valued field. Overall, we chose a now common point of view -- similar to that in \cite{CS19}-- which consists in seeing reduction to the $\RV$-sort simply as an intermediate step. The strategy is indeed to reduce to the $\RV$-sort and to continue the process of reduction later on, from the $\RV$-sort to the value group and residue field. Let us mention our reduction principle down to the $\RV$-sort.   

%A very important phenomenon, which creates quite some obstructions, is what
%is called non-well definability of the sum: one could have $\rv(a)=\rv(a')$
%and $\rv(b)=\rv(b')$ and $\rv(a+b) \neq \rv(a'+b')$. (This occurs exactly
%when $\rv(a) \oplus \rv(b)=0$.)




\textbf{Reduction to the $\RV$-sort.}



 We show that the $\RV$-sort of a benign valued field (see the list above) is as complex as the valued field itself with respect to the burden. 

{
    \renewcommand{\thetheorem}{\ref{ThmHensValuedFieldReductionRV}}
\begin{theorem} 
Let $\mathcal{K}$ be a benign valued field. Let $M$ be a positive integer. Then $\mathcal{K}$ is of burden $M$ if and only if the sort $\RV$ with the induced structure is also of burden $M$. In particular, $\mathcal{K}$ is inp-minimal if and only if $\RV$ is inp-minimal.
\end{theorem}
    \addtocounter{theorem}{-1}
    }



For stably embedded substructure, we got the following theorem:

{
    \renewcommand{\thetheorem}{\ref{PropRV}}

    \begin{theorem} Let $\mathcal{L}/ \mathcal{K}$ be a separated extension of valued fields, and assume that $Th(\mathcal{L})$ is a benign theory of Henselian valued field. The following are equivalent:
        \begin{enumerate}
            \item $K$ is stably embedded (resp.\ uniformly stably embedded) in $\mathcal{L}$ (in $\Th(\mathcal{L})$),
            \item $\RV_K$ is stably embedded (resp.\ uniformly stably embedded) in $\RV_L$.
        \end{enumerate}
    \end{theorem}

    \addtocounter{theorem}{-1}
    }
    
We also proved similar statements for mixed characterisitic Henselian valued fields. See Theorems \ref{ThmHensValuedFieldReductionRVMixedCharacteristic} and \ref{PropRV<omega}.

These reduction principles are possible due to the fact that benign valued fields
eliminate quantifiers relatively to the $\RV$-sort. In fact, our reduction of burden makes a decisive use of a slightly improved statement for one-dimensional definable set: every formula with one
free variable $x$ can be written in the following form:
\[\phi(\rv(x-a_0), \ldots , \rv(x-a_{n-1}), \beta)\]
where $\phi(x_0,\cdots,x_{n-1},\beta)$ is an $\RV$-formula. Notice that field-sorted terms are linear in $x$, and that a non-improved relative quantifier elimination result would only give polynomial field-sorted-terms). This result is due to Flenner in the case of characteristic $0$, but  we had to prove it in the general case of benign valued fields (see Theorem \ref{TheoremLinearTerms}).
 This has some intuitive consequences, allowing us for instance to picture the valued field as a tree and to let aside algebraic consideration such as roots of polynomial. At the same time, this dependence of a description of one dimensional definable sets adds a layer of difficulty and an obstacle to potential generalisation, notably to valued fields with generic automorphism.


\textbf{Resplendence of relative quantifier elimination.}\\
Quantifier elimination relative to a sort $S$ is said to be resplendent if it may be extended to any enrichment of the structure on $S$. This happens naturally and for syntactical reasons namely when the sort $S$ is `closed', meaning there is no function/predicate symbols from the sort $S$ to the rest of the structure. This is a well known fact
which has been formalised in \cite{Rid17}. All results of relative quantifier elimination in this text will be resplendent, and this notion will be intensively used through this text. In fact, all the main theorems cited above are resplendent -- we mean that they still hold after enrichment of the value group and residue field or the $\RV$-sort. This gives natural generalisations to richer theories and avoids unnecessary repetition  (`one may prove similarly that ... '). Resplendency is for instance used to extend relative results on valued fields to valued fields with $\ac$-map. One needs for that to notice that an $\ac$-map is an enrichment of the $\RV$-sort, and to treat the reduction from the $\RV$-sort to the value group $\Gamma$ and residue field $k$. The situation is then much simpler as the $\RV$-sort may be identified with the product $k\times \Gamma$. Notice however that an $\ac$-map is not an enrichment of neither the value group nor the residue field; a direct reduction to the value group and residue field would have not implied these statements.
\textit{A contrario}, working resplendently allows us to ignore `superficial structure' and therefore helps to simplify proofs and notations. 



\textbf{Reduction to the residue field and value group.}


    

As in \cite{CS19}, we see an $\RV$-sort of a `benign' valued field as an enriched short exact sequence 
\[1 \rightarrow k^\star \rightarrow \RV^\star \rightarrow \Gamma \rightarrow 0\]
of abelian groups. 
Let us consider first `benign' valued fields with an $\ac$-map $\ac:K^\star \rightarrow k^\star$. The situation become simpler: one sees that adding an $\ac$-map is equivalent to adding a spliting of the exact sequence above. By resplendence, it remains to reduce our problems from a product $k^\star\times \Gamma$ to $\Gamma$ and $k$. We were naturally lead to the following proposition and lemma:

    {
    \renewcommand{\thetheorem}{\ref{sumburden}}
   \begin{proposition}
    Let $\mathcal{K}$ and $\mathcal{H}$ be two structures, and consider the multisorted structure $\mathcal{G}$:
    \[\mathcal{G}=\{ K \times H, \mathcal{K},\mathcal{H}, \pi_K: K\times H \rightarrow K, \pi_H: K\times H \rightarrow H \},\]
    called the \emph{direct product structure} (where $\pi_K$ and $\pi_H$ are the natural projections). Then $\mathcal{G}$ eliminates quantifiers relative to $\mathcal{K}$ and $\mathcal{H}$, and $\mathcal{K}$ and $\mathcal{H}$ are orthogonal and stably embedded within $\mathcal{G}$. 

    We have $$\bdn(\mathcal{G}) = \bdn(\mathcal{K})+ \bdn(\mathcal{H}).$$
    \end{proposition}
    \addtocounter{theorem}{-1}
    }   
    
    {
    \renewcommand{\thetheorem}{\ref{LemmaProductStEmbSubstruc}}
    \begin{lemma} Let $\mathcal{H}_1$ (resp.\ $\mathcal{K}_1$) be a substructure of a structure $\mathcal{H}_2$ (resp.\ $\mathcal{K}_2$). Then $\mathcal{H}_1\times \mathcal{K}_1$ is a substructure of $\mathcal{H}_2\times \mathcal{K}_2$ and we have:
    \begin{itemize}
        \item $\mathcal{H}_1\times \mathcal{K}_1$ is stably embedded in $\mathcal{H}_2\times \mathcal{K}_2$ if and only if $\mathcal{H}_1$ is stably embedded in $\mathcal{H}_2$ and $\mathcal{K}_1$ is stably embedded in $\mathcal{K}_2$.
        \item $\mathcal{H}_1\times \mathcal{K}_1$ is uniformly  stably embedded in $\mathcal{H}_2\times \mathcal{K}_2$ if and only if $\mathcal{H}_1$ is uniformly  stably embedded in $\mathcal{H}_2$ and $\mathcal{K}_1$ is uniformly  stably embedded in $\mathcal{K}_2$.
    \end{itemize}
    \end{lemma}
    \addtocounter{theorem}{-1}
    }

    
    Naturally, the question of the reduction of benign valued fields without $\ac$-map requires more work, as one has to really deal with the structure of a short exact sequence $1 \rightarrow k^\star \rightarrow \RV^\star \rightarrow \Gamma \rightarrow 0$. By resplendence, we can forget the additive structure on the residue field, and the ordered structure on the value group. As the following results are interesting in their own, we leave the traditional notation of valued fields, and name our sequences of abelian groups $0 \rightarrow A \rightarrow B \rightarrow C \rightarrow 0$.


    {
    \renewcommand{\thetheorem}{\ref{ThmBdnExSeq}}
    \begin{theorem}
        Consider an $\{A\}$-$\{C\}$-enrichement of an exact sequence $\mathcal{M}$ of abelian groups
    \[ \xymatrix{0 \ar[r] & A \ar[r]^{\iota}& B \ar[r]^{\nu} & C\ar[r] &0}. \]
    Assume that $A$ is a pure subgroup of $B$: for all $a \in A$, $b \in B$ if $\iota(a)=nb$, then there is $a'\in A$ such that $a=na'$.
        We have 
        \[\bdn\mathcal{M} =\max_{n\in \mathbb{N}}(\bdn(A/nA)+\bdn(nC)).\]
        
        In particular, if $A/nA$ is finite for all $n\geq 1$, then \[\bdn{\mathcal{M}}= \max(\bdn(A), \bdn(C)).\]
    \end{theorem}
    \addtocounter{theorem}{-1}
    }   
    
    {
    \renewcommand{\thetheorem}{\ref{CorollaryStablyEmbeddedSubShortExactSequence}}
        \begin{corollary}
        Let $\mathcal{N} = \{0\rightarrow A \rightarrow B \rightarrow C \rightarrow 0\}$ be a (possibly $\{A\}$-$\{C\}$-enrichement of a) pure short exact sequence of abelian groups,  and let $\mathcal{M} \subseteq \mathcal{N}$ be a sub-short exact sequence. Assume either 
        \begin{itemize}
            \item that $C(\mathcal{M})$ is a pure subgroup of $C(\mathcal{N})$,
            \item or that $\rho_n^{\mathcal{N}}(\mathcal{M})$ is finite for all $n\geq 1$\footnote{we will denote by $\rho_n^{\mathcal{N}}(\mathcal{M})$ the image of $\mathcal{M}$ in $A/nA$ under a certain natural projection map. The condition is in particular satisfied if $A/nA$ is itself finite}. 
       \end{itemize}
        Then, we have:
        \begin{itemize}
        	\item  $\mathcal{M} $ is stably embedded in $\mathcal{N}$ if and only if $A(\mathcal{M})$ is stably embedded in $A(\mathcal{N})$ and $C(\mathcal{M})$ is stably embedded in $C(\mathcal{N})$,
        	\item  $\mathcal{M} $ is uniformly stably embedded in $\mathcal{N}$ if and only if $A(\mathcal{M})$ is uniformly stably embedded in $A(\mathcal{N})$ and $C(\mathcal{M})$ is uniformly stably embedded in $C(\mathcal{N})$.
\end{itemize}
    \end{corollary}
    \addtocounter{theorem}{-1}
    }
    
    
    
    
Is the study of the $\RV$-sort necessary? It is at least very convenient and seems canonical in a certain way: the $\RV$-sort seems to be the least substructure within benign valued fields containing the value group and residue field and where reduction principles apply. And as we saw, it also has the advantage to generalise in the context of valued fields with an $\ac$-map. \\



\textbf{ Organisation of the text }\\
A large part of this text is dedicated to preliminaries in Chapter \ref{ChapterPreliminaries}. In Section \ref{SectionOnPureModelTheory}, we define pure model theoretic notions such as burden and stable embeddedness. In Section \ref{SectionModelTheoryAlgebraicStructures}, we describe essential model theoretic properties of algebraic structures: valued fields and short exact sequences of abelian groups. It also includes important lemmas and propositions. \\
We prove our transfer principles for burden in Chapter \ref{ChapterBurden}, which is split in four sections: in Section \ref{SectionReductionBurdenRV} we treat the reduction to the $\RV$-sort, in Section \ref{SectionExactSequence} the reduction in pure short exact sequences of abelian groups, in Section \ref{SectionHenselianValuedFieldsEquichar0} the reduction to the value group and residue field for benign valued fields, and in Section \ref{SectionUnrimified} the reduction to the value group and residue field for unramified mixed characteristic Henselian valued fields with perfect residue field.\\
We treat then our transfer principles for stably embedded pairs of valued fields in Chapter \ref{ChapterStablyEmbeddedPairs}. For some technical reason, this chapter has a slightly different structure. It is split in three sections: Section \ref{SectionReductionStableEmbeddednessBenignValuedFields} treats the reduction in the context of benign valued fields and Section \ref{SectionReductionStableEmbeddednessUnramifiedMixedCharacteristic} treats the reduction in the context of unramified mixed characteristic Henselian valued fields with perfect residue field. In both sections, we reduce first to the $\RV$-sort. In the first, we provide a transfer principle for stably embedded pairs of pure short exact sequences. Then, in Section \ref{SectionPairs}, we treat as a corollary the elementarity of the class of stably embedded elementary pairs of benign valued fields.

The reader will also find some sparse results. For instance, we took the opportunity to briefly study and construct non-uniformly stably embedded pairs of random graphs in Appendix \ref{OnPairsOfRandomGraphs}. In Appendix \ref{LexicographicProduct}, we produce a transfer principle for burden in Lexicographic products. We also gave an attempt in Subsection \ref{More on burden and strongness} to formalise and justify a common convention which consists of writing $\bdn(T)\leq \aleph_{0-}$ if a theory $T$ is strong.\\


